Learning a Metric Embedding for Face Recognition using the Multibatch Method

This work is motivated by the engineering task of achieving a near state-of-the-art face recognition on a minimal computing budget running on an embedded system. Our main technical contribution centers around a novel training method, called Multibatch, for similarity learning, i.e., for the task of generating an invariant "face signature" through training pairs of "same" and "not-same" face images. The Multibatch method first generates signatures for a mini-batch of $k$ face images and then constructs an unbiased estimate of the full gradient by relying on all $k^2-k$ pairs from the mini-batch. We prove that the variance of the Multibatch estimator is bounded by $O(1/k^2)$, under some mild conditions. In contrast, the standard gradient estimator that relies on random $k/2$ pairs has a variance of order $1/k$. The smaller variance of the Multibatch estimator significantly speeds up the convergence rate of stochastic gradient descent. Using the Multibatch method we train a deep convolutional neural network that achieves an accuracy of $98.2\%$ on the LFW benchmark, while its prediction runtime takes only $30$msec on a single ARM Cortex A9 core. Furthermore, the entire training process took only 12 hours on a single Titan X GPU.

==> pairs-vs-all-pairs.tex <==
% This file was created by matplotlib2tikz v0.5.4.
% The lastest updates can be retrieved from
% 
% https://github.com/nschloe/matplotlib2tikz
% 
% where you can also submit bug reports and leavecomments.
% 
\begin{tikzpicture}

\begin{axis}[
xmin=0, xmax=1000000,
ymin=0, ymax=1000000,
axis on top,
width=\figurewidth,
height=\figureheight
]
\addplot [red, mark=*, mark size=3, mark options={draw=black}, only marks]
table {%
874161 193708
874161 245920
874161 310304
874161 552095
874161 593006
874161 599570
874161 629518
874161 684468
874161 770102
806292 245920
806292 310304
806292 552095
806292 593006
806292 599570
806292 629518
806292 684468
806292 770102
754080 310304
754080 552095
754080 593006
754080 599570
754080 629518
754080 684468
754080 770102
689696 552095
689696 593006
689696 599570
689696 629518
689696 684468
689696 770102
447905 593006
447905 599570
447905 629518
447905 684468
447905 770102
406994 599570
406994 629518
406994 684468
406994 770102
400430 629518
400430 684468
400430 770102
370482 684468
370482 770102
315532 770102
};
\addplot [black, mark=diamond*, mark size=3, only marks]
table {%
874161 593006
806292 599570
754080 629518
689696 684468
447905 770102
};
\end{axis}

\end{tikzpicture}
